The basic reproduction number, $R_0$, in structured populations

In this paper, we provide a straightforward approach to defining and deriving the key epidemiological quantity, the basic reproduction number, $R_0$, for Markovian epidemics in structured populations. The methodology derived is applicable to, and demonstrated on, both $SIR$ and $SIS$ epidemics and allows for population as well as epidemic dynamics. The approach taken is to consider the epidemic process as a multitype process by identifying and classifying the different types of infectious units along with the infections from, and the transitions between, infectious units. For the household model, we show that our expression for $R_0$ agrees with earlier work despite the alternative nature of the construction of the mean reproductive matrix, and hence, the basic reproduction number.

==> intro.tex <==
\section{Introduction} \label{S:intro}

The basic reproduction number, $R_0$, is a key summary in infectious disease modelling being defined as the expected number of individuals infected by a typical individual in a completely susceptible population. This definition of $R_0$ is straightforward to define and compute in a homogeneous population consisting of a single type of infective (homogeneous behaviour) and with uniform random mixing of infectives (homogeneous mixing). This yields the celebrated threshold theorem, see for example, \cite{Whittle55}, for the epidemic with a non-zero probability of a major epidemic outbreak if and only if $R_0 >1$.

The extension of the definition $R_0$ to non-homogeneous populations is non-trivial. Important work in this direction includes \cite{Diekmann_etal} which considers heterogeneous populations consisting of multiple types of infectives and \cite{Pellis_etal}, \cite{Ball_etal} which consider heterogeneity in mixing through population structure. Specifically \cite{Diekmann_etal} defines for a population consisting of $K$ types of infectives, the $K \times K$ mean reproduction matrix $\mathbf{M}$ (also known as the next-generation-matrix), where $M_{ij}$ denotes the mean number of infectives of type $j$ generated by a typical type $i$ infective during its infectious period. Then $R_0$ is defined as the Perron-Frobenius (dominant) eigenvalue of $\mathbf{M}$. By contrast \cite{Pellis_etal} and \cite{Ball_etal} focus on a household epidemic model with a single type of infective and consider a branching process approximation for the initial stages of the epidemic process, see, for example, \cite{Whittle55}, \cite{Ball_Donnelly} and \cite{BMST}. \cite{Pellis_etal} consider the asymptotic growth rate of the epidemic on a generational basis using an embedded Galton-Watson branching process and define $R_0$ to be
\begin{eqnarray} \label{eq:intro:1} R_0 = \lim_{n \rightarrow \infty} \ez [X_n]^{1/n}, \end{eqnarray}
where $X_n$ is the number of infectives in the $n^{th}$ generation of the epidemic. Given that the mean reproduction matrix $\mathbf{M}$ represents the mean number of infectives generated by an infective in the next generation, we observe that the computation of $R_0$ in both cases is defined in terms of the generational growth rate of the epidemic.

The current work applies the approach of \cite{Diekmann_etal} to Markovian epidemics in structured populations and thus assumes individuals have exponentially distributed infectious periods. Using the method of stages \cite{Barbour76} it is straightforward to extend the work to more general infectious periods consisting of sums or mixtures of exponential random variables. Alternatively by considering the epidemic on a generational basis in the spirit of \cite{Pellis_etal} we can adapt our approach to general infectious periods for $SIR$ or $SEIR$ epidemics. Note that as demonstrated in a sexually transmitted disease example in Section \ref{S:example:sex}, our approach applies to $SIS$ epidemics as well. The key idea is that in structured populations we can define infectives by the type of infectious unit to which they belong, where for many models the number of type of infectious units is relatively small and easy to classify. By characterising an infective by the type of infectious unit they originate in (belong to at the point of infection) and considering the possible events involving the infectious unit, we can write down a simple recursive equation for the mean reproduction matrix $\mathbf{M}$. Then as in \cite{Diekmann_etal} we can simply define $R_0$ to be the Perron-Frobenius eigenvalue of $\mathbf{M}$. 

Our approach is similar to \cite{LKD15}, who also consider classifying infectives by the type of infectious unit to which they belong in an dynamic $SI$ sexually transmitted disease model which is similar to the $SIS$ model studied in Section \ref{S:example:sex}. The modelling in \cite{LKD15} is presented in a deterministic framework with \cite{Lashari_Trapman} considering the model from a stochastic perspective. The key difference to \cite{LKD15} is that we work with the embedded discrete Markov process of the transition events rather than the continuous time Markov rate matrices. The advantages of studying the discretised process is that it is easier to incorporate both local (within-infectious unit) infections and global (creation of new infectious units) infections and in generalisations of the construction of $\mathbf{M}$ beyond exponential infectious periods, see Section \ref{S:example:gcm} and Appendix \ref{App:rank}.

The remainder of the paper is structured as follows. In Section \ref{S:setup} we define the generic epidemic model which we consider along with the derivation of $\mathbf{M}$ and $R_0$. To assist with the understanding we illustrate with an $SIR$ household epidemic model (\cite{BMST}, \cite{Pellis_etal} and \cite{Ball_etal}). In Section \ref{S:Example}, we detail the computing of  $\mathbf{M}$ and $R_0$, for the $SIR$ household epidemic model (Section \ref{S:example:house}), an $SIS$ sexually transmitted disease model (Section \ref{S:example:sex}), see, for example, \cite{Kret}, \cite{LKD15} and \cite{Lashari_Trapman} and the great circle $SIR$ epidemic model (Section \ref{S:example:gcm}), see \cite{BMST}, \cite{Ball_Neal02} and \cite{Ball_Neal03}. In Section \ref{S:example:house} we show that the computed $R_0$ agrees with $R_0^g$ obtained in \cite{Ball_etal}.



% Add generational construction of events for $SIR$ dynamics where population structure does not change. More generally where individuals move between structures -ie. relationship this does not hold.
%
%
%

